A Survey on Hypergraph Neural Networks: An In-Depth and Step-By-Step Guide

Higher-order interactions (HOIs) are ubiquitous in real-world complex systems and applications. Investigation of deep learning for HOIs, thus, has become a valuable agenda for the data mining and machine learning communities. As networks of HOIs are expressed mathematically as hypergraphs, hypergraph neural networks (HNNs) have emerged as a powerful tool for representation learning on hypergraphs. Given the emerging trend, we present the first survey dedicated to HNNs, with an in-depth and step-by-step guide. Broadly, the present survey overviews HNN architectures, training strategies, and applications. First, we break existing HNNs down into four design components: (i) input features, (ii) input structures, (iii) message-passing schemes, and (iv) training strategies. Second, we examine how HNNs address and learn HOIs with each of their components. Third, we overview the recent applications of HNNs in recommendation, bioinformatics and medical science, time series analysis, and computer vision. Lastly, we conclude with a discussion on limitations and future directions.

==> 900Abstract.tex <==

Group interactions are ubiquitous, and hypergraphs naturally express such interactions. 
Hypergraph representation learning has demonstrated its effectiveness for related downstream tasks, especially compared to graph representation learning.
Despite the rising attention to hypergraph representation learning, there has been no broad tutorial to provide its overview. 
As such, we provide a timely tutorial on hypergraph representation learning, with a focus on their models, training strategies, and recent applications.
We {conclude} the tutorial with a discussion on {current} frontiers and open problems.

==> 901Basic.tex <==
\begin{comment}
We provide an overview of hypergraph representation learning, 
focusing on hypergraph neural networks, training strategies, and their applications.
The expected length of the tutorial is two hours.
\end{comment}

We provide the first tutorial on hypergraph neural networks (HNNs), focusing on an in-depth and step-by-step analysis of (a) each component of HNNs, (b) training strategies of HNNs, and (c) applications of HNNs.
The expected length of the tutorial is three hours.

==> 902Motivation.tex <==
\smallsection{Motivation and Significance}
% About hypergraphs
Hypergraphs are widely adopted to model higher-order interactions among multiple entities, which are natural and prevalent. 
Examples include collaboration of researchers, co-purchase of items, and joint interaction among proteins.
%Advantages of a hypergraph over a graph
Modeling such higher-order interactions as an ordinary graph with pairwise edges is suboptimal with potential information loss~\cite{do2020structural,dong2020hnhn}.
As a result, {hypergraphs} have gained attention in various domains, including recommender systems~\cite{xia2021self, wang2021session}, finance~\cite{sawhney2021stock, sawhney2020spatiotemporal}, biomedicine~\cite{saifuddin2023hygnn}, %ruan2021exploring
and sociology~\cite{sun2023self}.
Interest in hypergraph representation learning, particularly hypergraph neural networks (HNNs), has also been rapidly rising. 
Notably, HNNs, a class of neural networks designed to operate on hypergraphs, have led to substantial performance improvement over graph neural networks in various downstream tasks, including node classification~\cite{feng2019hypergraph}, edge prediction~\cite{yadati2020nhp}, and clustering~\cite{lee2023m}.
Therefore, we aim to provide a timely tutorial on hypergraph neural networks, with our primary focus on their components, training strategies, and {real-world} applications. \\

\smallsection{Targeted Audience and Prerequisites}
%Target
This tutorial is intended for researchers and practitioners who are interested in representation learning for higher-order interactions and its significant applications, including recommender systems. 
%Prerequisite
We expect that the audience is familiar with some basic concepts and terminologies of data mining and artificial intelligence, such as neural networks and their training methods. 
{Specialized} engineering skills are not required to understand the tutorial, but a preliminary understanding of graph representation learning, especially graph neural networks, would be beneficial.
%Expected benefit
Throughout the tutorial, the audience will gain insights into hypergraph representation learning methods and their applications, {including their advantages, unique challenges, and novel solutions compared to graph representation learning.}

%This tutorial may offer new insights for research and application.
%Informal evidence that people would attend


==> 903Outline.tex <==
We provide an in-depth and step-by-step guide to hypergraph neural networks, focusing on their
(1) components, 
(2) training strategies, 
(3) applications, and
(4) open problems and frontiers.

\begin{itemize}[leftmargin=*]

    \item \textbf{Part I: Introduction} (10 mins)
    \begin{itemize}
        \item Modeling higher-order interactions as hypergraphs
        \item Public hypergraph datasets
        \item {Comparison with graph modeling}
    \end{itemize}
    
    \item \textbf{Part II: Components of HNNs} (60 mins)
    \begin{itemize}
        \item Overview of hypergraph neural networks
    
        \item \underline{\smash{(C1) Feature design}}, focusing on  external features~\cite{yadati2019hypergcn, chien2021you, kim2023datasets} and structural features~\cite{huang2019hyper2vec, choe2023classification, saifuddin2023topology}
        
        \item \underline{\smash{(C2) Hypergraph expression}}, focusing on clique expansion~\cite{feng2019hypergraph, tang2024hypergraph}, adaptive expansion~\cite{yadati2019hypergcn, qian2023adaptive2}, star expansion~\cite{wang2022equivariant, chien2021you}, and line expansion~\cite{yang2022semi}

        \item \underline{\smash{(C3) Message passing}}, focusing on target selection (single~\cite{prokopchik2022nonlinear, wang2023hypergraph} or multi~\cite{saifuddin2023hygnn, gao2022hgnn+} stages), message representation (hyperedge-consistent~\cite{huang2021unignn, dong2020hnhn} or hyperedge-dependent~\cite{choe2023classification, telyatnikov2023hypergraph}), and message aggregation (fixed~\cite{wang2024dynamic, wang2022equivariant} or adaptive~\cite{chien2021you, bai2021multi} pooling)
    \end{itemize}

    \item \textbf{Part III: Training strategies for HNNs} (60 mins)
    \begin{itemize}
        \item \underline{\smash{(T1) Learning to classify}}, focusing on rule-based and learnable negative sampling~\cite{yadati2020nhp, patil2020negative, hwang2022ahp, ko2023enhancing}

        \item \underline{\smash{(T2) Learning to contrast}}, focusing on augmentation schemes and loss functions~\cite{lee2023m, wei2022augmentations, kim2023datasets, qian2023adaptive}

        \item \underline{\smash{(T3) Learning to generate}}, focusing on self-supervision~\cite{kim2023hypeboy, du2022self} and structural learning \cite{cai2022hypergraph, lei2024unveiling}
    \end{itemize}
    
    \item \textbf{Part IV: Applications of HNNs} (30 mins)
    \begin{itemize}
        \item \underline{\smash{(A1) Recommendation}}~\cite{li2021hyperbolic, li2022enhancing,xia2022self, xia2021self}
        \item \underline{\smash{(A2) Bioinformatics and medical science}}~\cite{chen2023teasing, liu2022multi, wang2024dynamic, wu2023megacare}
        \item \underline{\smash{(A3) Time series analysis}}~\cite{wang2023dynamic, yi2020hypergraph, li2022spatial, liao2024stock}
        \item \underline{\smash{(A4) Computer vision}}~\cite{bai2021multi, liu2020semi, xu2022adaptive, yan2020learning}
    \end{itemize}
    
    \item \textbf{Part V: Open problems and frontiers} (20 mins)
    \begin{itemize}
        \item Theoretical analysis on HNNs~\cite{luo2023expressiveness, hayhoe2023transferable}
        \item Necessity of HNNs~\cite{yoon2020much}
        \item HNNs for complex hypergraphs~\cite{luo2022directed, agarwal2022think}
    \end{itemize}
\end{itemize}


==> 904Tutors.tex <==
\textbf{Sunwoo Kim (in-person presenter) is a Ph.D. student at Kim Jaechul Graduate School of AI, KAIST, South Korea.}
He received his M.S. degree in artificial intelligence from KAIST in 2024 and B.A. degree in applied statistics from Yonsei University in 2022.
His research interests include hypergraph representation learning and mining. 
His works have been published in major venues, including KDD, ICDM, ICLR, and CVPR. 
More information about Sunwoo can be found at \url{https://sites.google.com/view/sunwoo97}.
\\

\noindent\textbf{Soo Yong Lee (in-person presenter) is a Ph.D. student at Kim Jaechul Graduate School of AI, KAIST, South Korea.}
He received his M.S. degree in artificial intelligence from KAIST in 2023 and B.S. degree in psychology from UCSD in 2016.  
His research interests include (hyper)graph representation learning and mining. 
His works have been published in major venues, including WWW, CIKM, ICML, and ICLR. 
More information about Soo Yong can be found at \url{https://github.com/syleeheal/}.
\\

\noindent\textbf{Yue Gao (in-person presenter) is a Tenured Associate Professor at the School of Software, Tsinghua University, China.}
He received his Ph.D. from the Department of Automation at Tsinghua University in 2012.
His research falls in the fields of AI, CV, and brain science. 
He has published 100+ papers in premier conferences and journals, including KDD, CVPR, and TPAMI. 
%He also serves as an editorial board member/associate editor for the International Journal of Computer Vision and Medical Image Analysis. 
More information about Yue can be found at \url{https://www.thss.tsinghua.edu.cn/en/faculty/yuegao.htm}.
%He is a Senior Member of IEEE and a Member of ACM. 
\\

\noindent\textbf{Alessia Antelmi (in-person presenter) is an Assistant Professor at the Department of Computer Science of the University of Turin, Italy.} She received her MSc and Ph.D. in Computer Science from the University of Salerno (Italy) in 2018 and 2022, respectively. 
%In 2018, Alessia got a student travel grant to visit the Unit for Social Semantics, Data Science Institue (Galway, Ireland), led by Prof. John Breslin, and, in 2023, a research grant to join the NERDS research group at ITU to work on the COCOONS project led by Prof. Luca Maria Aiello. 
Her research primarily relates to exploiting hypergraphs to study the high-order relationships characterizing real-world phenomena, %, specifically focusing on online social influence diffusion and collective behavior
More information about Alessia can be found at \url{https://alessant.github.io/}. \\


\noindent\textbf{Mirko Polato (contributor) is an Assistant Professor at the Department of Computer Science of the University of Turin, Italy.} 
Mirko Polato received his Ph.D. in Brain, Mind, and Computer Science from the University of Padova (Italy) in 2018. 
%In 2017, Dr. Polato was a visiting Ph.D. student at the Delft University of Technology in the Multimedia Computing group.
%From 2018 to 2021, he was a post-doctoral fellow at the University of Padova, working on two H2020 projects. Since 2021, he has been an Assistant Professor at the University of Turin, and 
His main research topics include federated learning, interpretable machine learning, hypergraph representation learning, and recommender systems.
%He co-organized Special Sessions and Workshops on many top venues, including WWW and IJCNN.
%He served as a Program Committee member of several international conferences and as a referee for several international journals. 
He authored about 50 research products, including international peer-reviewed conferences and journal papers.
More information about Mirko can be found at \url{https://makgyver.github.io}. \\

\noindent\textbf{Kijung Shin (in-person presenter) is an Associate Professor jointly affiliated in the Kim Jaechul Graduate School of AI and the School of Electrical Engineering at KAIST, South Korea.} He received his Ph.D. in Computer Science from Carnegie Mellon University (USA) in 2019.  
His research interests span various topics on data mining and machine learning for (hyper)graph-structured data, with a focus on scalable algorithm design and empirical patterns in the real world. He has published more than 70 referred articles in major data mining, database, and machine learning venues. He won the best research paper award at KDD 2016 and the best student paper runner-up award at ICDM 2023. 
More information about Kijung can be found at \url{https://kijungs.github.io}. \\

\noindent The \textbf{corresponding tutor} is Kijung Shin (email: kijungs@kaist.ac.kr and tel: +82-958-3915).

==> 905SimilarTutorial.tex <==
\smallsection{Graph Representation Learning}
Several tutorials focusing on graph representation learning were delivered in KDD and other data-mining venues, including one by~\citet{grltutorial} at KDD 2021 on August 14.
Although these tutorials focus on {ordinary graphs with \textit{pairwise interactions}}, 
the {proposed} tutorial focuses on hypergraphs that express \textit{higher-order interactions} among an arbitrary number of entities.
{Note that modeling such higher-order interactions as ordinary graphs is suboptimal with potential information loss~\cite{dong2020hnhn,do2020structural}}, which may risk hypergraph neural networks to suffer from performance degradation in various downstream tasks (e.g. node classification~\cite{feng2019hypergraph}, edge prediction~\cite{yadati2020nhp}, and clustering~\cite{lee2023m}).

\smallsection{Hypergraph Mining}
A previous tutorial on hypergraph mining was conducted by one of the tutors~\citep{lee2022mining} at several venues, including KDD 2023 in Long Beach, CA, USA, on August 6.
This previous tutorial focuses on mining and reproducing empirical patterns in real-world hypergraphs.
The proposed tutorial, however, focuses on hypergraph neural networks.
\textbf{Note that there is minimal overlap, with no key references shared in both tutorials.}
The slides used for the previous tutorial are available at {\url{https://sites.google.com/view/hypergraph-tutorial}}.

\begin{comment}
\smallsection{Graph Representation Learning}
{Previous tutorials on graph representation learning focus on {ordinary graphs with \textit{pairwise interactions}}.\footnote{\url{http://cse.msu.edu/~mayao4/tutorials/aaai2020/}} \footnote{\url{http://snap.stanford.edu/proj/embeddings-www/}}} 
The {proposed} tutorial, however, focuses on hypergraphs that express \textit{group interactions} among an arbitrary number of entities.
{Note that modeling such group interactions as ordinary graphs is suboptimal with potential information loss~\cite{dong2020hnhn,do2020structural}}, which may risk the representation learning models to suffer from performance degradation in various downstream tasks (e.g. node classification~\cite{feng2019hypergraph}, edge prediction~\cite{yadati2020nhp}, and clustering~\cite{lee2023m}).

\smallsection{Hypergraph Mining}
A previous tutorial on hypergraph mining \cite{lee2022mining} focus on mining and reproducing patterns in real-world hypergraphs.\footnote{\url{https://sites.google.com/view/hypergraph-tutorial}}
The proposed tutorial, however, focuses on representation learning on hypergraphs.
Note that there is minimal overlap, with fewer than five shared references between the two tutorials.
\end{comment}

==> 906Interactivity.tex <==
\smallsection{Online Q\&A}
We plan to leverage an online Q\&A platform like Slido throughout the tutorial.\footnote{\url{https://www.slido.com/features-live-qa}}
The audience can freely and comfortably submit questions at any time.
Moreover, by facilitating anonymous questions—a feature supported by Slido—we aim to create a more comfortable %and informal 
environment for the audience to pose their queries.
We intend to schedule brief Q\&A sessions between subtopics to address both pre-submitted (online) and live (offline) questions, ensuring %a comprehensive and
interactive learning experience.

\smallsection{Illustraion and examples}
Understanding the lecture content is essential for effective interaction, so we will dedicate considerable effort to ensuring the audience fully grasps the content. 
To achieve this, we will employ illustrations and examples to clarify every concept covered in the tutorial. 
This is particularly crucial for describing hypergraph neural network architectures, where we intend to offer a comprehensive visual explanation of each step involved in message passing, alongside ample intuition into each component.

==> 907Impact.tex <==
Higher-order interactions are pervasive across numerous domains, and hypergraphs are widely adopted in analyzing these complex relationships. 
In line with this trend, hypergraph neural networks (HNNs) are evolving to be more strong and intricate within the fields of data mining and machine learning. 
However, their increasing complexity poses a significant barrier to non-experts aspiring to utilize cutting-edge models. 
Our tutorial is designed to demystify HNNs for individuals from diverse disciplines, facilitating a smoother adoption of sophisticated models. 
Furthermore, by comprehensively addressing each component of HNNs, we hope to enable participants to develop their custom HNNs, %tailored to their specific needs, 
ultimately broadening the application and innovation in this field.
